Traffic signal optimization: combining static and dynamic models

In this paper, we present a cyclically time-expanded network model for simultaneous optimization of traffic assignment and traffic signal parameters, in particular offsets, split times, and phase orders. Since travel times are of great importance for developing realistic solutions for traffic assignment and traffic signal coordination in urban road networks, we perform an extensive analysis of the model. We show that a linear time-expanded model can reproduce realistic travel times especially for use with traffic signals and we verify this by simulation. Furthermore, we show how exact mathematical programming techniques can be used for optimizing the control of traffic signals. We provide computational results for real world instances and demonstrate the capabilities of the cyclically time-expanded by simulation results obtained with state-of-the-art traffic simulation tools.

==> cyclic_discussion.tex <==
\subsection{travel times }

higher dimension, linear $\Rightarrow$ cool

\subsection{impact}

three to four \% compared to the best random solution or the consecutive approach.  However, thinking in absolute values, optimized offsets can already save about 10 hours of delay in every peak. Only 50 \% of the demand were measured 2 peaks per day and 250 working days per year, this adds up to 10.000 hours per year.  

\subsection{Future work}




One main question is the influence of traffic signal optimization on user equilibria. In a network without signals, system optimum and user equilibrium may look quite different. Does our method of optimizing signals and assignment push the equilibrium flow towards the system optimum flow by privileging the routes of the system optimum with progressive signal settings and penalizing the bad links of the user equilibrium with high waiting times?





short comings
no user equilibrium 
no fifo
gap hard to close
